Elastic Product Quantization for Time Series

Analyzing numerous or long time series is difficult in practice due to the high storage costs and computational requirements. Therefore, techniques have been proposed to generate compact similarity-preserving representations of time series, enabling real-time similarity search on large in-memory data collections. However, the existing techniques are not ideally suited for assessing similarity when sequences are locally out of phase. In this paper, we propose the use of product quantization for efficient similarity-based comparison of time series under time warping. The idea is to first compress the data by partitioning the time series into equal length sub-sequences which are represented by a short code. The distance between two time series can then be efficiently approximated by pre-computed elastic distances between their codes. The partitioning into sub-sequences forces unwanted alignments, which we address with a pre-alignment step using the maximal overlap discrete wavelet transform (MODWT). To demonstrate the efficiency and accuracy of our method, we perform an extensive experimental evaluation on benchmark datasets in nearest neighbors classification and clustering applications. Overall, the proposed solution emerges as a highly efficient (both in terms of memory usage and computation time) replacement for elastic measures in time series applications.

==> chapters/05-use_case.tex <==
\section{Use Case: Real-time recognition of handwritten Latex symbols}
Detexify\footnote{\url{https://detexify.kirelabs.org/classify.html}} is an online tool for recognizing hand-written LaTeX symbols~\cite{kirsch2010detexify}. It attempts to simplify the search for the LaTeX code of any symbol by allowing the user to sketch it. Since a user could draw faster or slower, template matching together with DTW is best suited to identify the corresponding LaTeX symbol. However, to deliver real-time performance, the classification is currently done with Euclidean distance \note{actually, it uses a greedy version of DTW} instead of DTW~\cite{kirsch2010detexify_git}. This is possible due to a large library of examples. In this section we justify PQDTW by showing how it improves the accuracy and performance in this real data mining task.

We use Detexify's public training data\footnote{The dataset can be downloaded from \url{https://github.com/kirel/detexify-data}} to train and evaluate our classifier. It contains 207,906 example strokes for 838 LaTeX symbols. The number of examples varies per symbol ($248.1\ \textrm{mean} \pm 416.3\ \textrm{std} $) and many examples are random scribbles rather than accurate sketches of the symbol. Each stroke is represented by an ordered series of coordinates and timestamps.

The strokes are first preprocessed and normalized. 
%We both consider a 2D and 1D representation. For the 2D representation, the strokes are shifted and scaled so that they are centered while maintaining their aspect ratio and maximally fill the square $[0, 1] \times [0, 1]$. Next, points with little curvature that do not add much to the characteristics of a stroke are filtered out. A critical angle $\alpha = 15^{\circ}$ is defined and the points at which the direction of the line changes by more than $\alpha$ are retained. This reduction in the number of points also speeds up DTW slightly.
To obtain a 1D representation of a stroke, each 2D point is replaced by the angle in relation to the next point in the stroke. 
Next, the 1D representation is smoothed and redistributed.
%Finally, both the 2D and 1D representation are smoothed and redistributed. 
Each point of a stroke is replaced by the arithmetic mean of the point and its two neighboring points. The points are redistributed so that the spatial distance between successive points is evenly large. The start and end points of lines are preserved. Golubitsky and Watt~\cite{golubitsky2009onlinecr} state that such a distribution of the points is actually the best choice when using DTW.

\begin{table}[]
\small
\caption{Results}
\begin{tabular}{llllll}
\toprule
       &         & \multicolumn{4}{c}{\bf Accuracy on top K} \\ 
{\bf Method} & {\bf Runtime} & {\bf Top 1}   & {\bf Top 3}   & {\bf Top 10}  & {\bf Top 20}  \\ \midrule
1D ED    & 21.5 ms ± 29.6 µs & 44.51   & 64.24   & 83.58   & 91.99   \\
%2D DTW   & 36.6 ms ± 724 µs  & 55.01   & 73.23   & 87.80   & 95.26   \\
1D DTW   & 709 ms ± 378 µs   & 45.94   & 68.55   & 87.83   & 95.50   \\
PQDTW   & 20.9 ms ± 31.2 µs & 43.82   & 64.09   & 85.26   & 93.82   \\ \bottomrule
\end{tabular}
\end{table}


Enables data mining tasks that require time warping and could not have been performed using time warping distance functions without the speedup provided by PQDTW.

==> chapters/06-related_work.tex <==
\section{Related work}

This paper proposed an adaptation of the PQ for Euclidean distance algorithm~\cite{jegou2010pq} to reduce the computational cost and memory footprint of DTW-based time series data mining algorithms. A naive adaptation of PQ for DTW was recently proposed by Zhang et al.~\cite{zhang2021}. They do not correct the unwanted alignments caused by the creation of subspaces. 

As already touched upon in Section~1, four alternative approaches are commonly used to mitigate the quadratic computational cost of DTW: constraint bands or warping windows~\cite{itakura1975,sakoe1978}, lower-bound pruning~\cite{kim2001lbkim,keogh2005lbkeogh,shen2018lbnew,lemire2009lbimproved,tan2019elastic,rakthanmanon2012lbcascade}, pruning warping alignments~\cite{silva2016pruneddtw}, and DTW approximations~\cite{salvador2007fastdtw,spiegel2014ltw}. In this work, we have shown how these existing techniques can be combined with PQ.

Thanks to the aforementioned DTW optimizations, the CPU usage of DTW is no longer the main constraint~\cite{rakthanmanon2012lbcascade}. Instead, disk I/O tends to be the bottleneck for the contemporary million-scale datasets that do not fit in main memory. Similar to the approach proposed in this paper, there have been numerous research efforts that propose to facilitate time series analysis by discretizing (i.e., symbolizing, tokenizing or quantizing) the raw data~\cite{daw2003:symbolization,andre1997,huang1999,megalooikonomou2005,shieh2008:isax}. These approaches first transform the raw data to a compact representation, which will fit in main memory, yet retains the essential features of the signal. The suggested approaches include general dimensionality reduction techniques such as Singular Value Decomposition (SVD)~\cite{chakrabarti2002:SVD}, Discrete Fourier Transform (DFT)~\cite{faloutsos1994:DFT}, and Discrete Wavelet Transform (DWT)~\cite{chang99:DWT}. Other approaches are based on piecewise approximations. Especially, the piecewise aggregate approximation (PAA)~\cite{keogh2001PAA,keogh2005PAAexact,shieh2008:isax} has been applied successfully. This representation divides each sequence into $k$ segments of equal length and represents each segment by its average value. The PAA has the beneficial property of lower-bounding the Euclidean distance, such that false dismissals are avoided. Though, there may be a lot of false alarms which may decrease the efficiency of retrieval and which could be problematic if the original dataset cannot be stored. Through quantization, a closer approximation of the original time series can be obtained. This idea has been applied to obtain a piecewise approximation of time series based on Euclidean distance~\cite{megalooikonomou2004}. To the best of our knowledge, no piecewise approximations exist that are based on DTW and allow shifting in the time axis.

%Beyond DTW, statistical-based approaches use measures that summarize characteristics or portions of time series (i.e., shapelets) as descriptive features to compare time series. \wm{Good to refer to but also mention that they are used to identify frequent patterns and not to obtain a similarity measure (thus rather to obtain features). Maybe also mention TSFresh as a feature based method to describe time series.}

%Shape segmented DTW:
%\begin{itemize}
%    \item Split sequences based on peaks (\url{https://doi.org/10.1007/978-3-030-20915})
%    \item Split sequences based on where they meet (\url{https://cgi.csc.liv.ac.uk/~frans/PostScriptFiles/sgai_Alshehri_2019.pdf})
%    \item Split sequences based on domain knowledge. For example, ECG data can be segmented  by  the  PQRST  chunks.
%\end{itemize}

==> media/algo_distance.tex <==
\begin{algorithm2e}[h]
\SetAlgoLined
\KwIn{\newline
$T_1$: A time series $ \in \mathbb{R}^{D}$\newline
$T_2$: A time series $ \in \mathbb{R}^{D}$\newline
$C$: the codebook $\in \mathbb{R}^{M \times k \times D/M}$\newline
$D$: the distance lookup table $\in \mathbb{R}^{M \times k \times k}$\newline
$E$: the Keogh envelopes $\in \mathbb{R}^{2 \times M \times k \times D/M}$
}
\KwOut{\newline
$d$: the distance between $T_1$ and $T_2$ $\in \mathbb{R}$\newline
}

$T_{1,enc} \gets \textbf{encode}(T_1, C, E)$\; 
$T_{2,enc} \gets \textbf{encode}(T_2, C, E)$\;

\SetKwProg{Fn}{Function}{ is}{end}
\Fn{symmetric($T_{1,enc}$,\ $T_{2,enc}$,\ $D$) : $\mathbb{R}$}{
    $dist \gets 0$\;
    \For{$m \gets 0$ \textbf{to} $M$} {
        $c_1 \gets T_{1,enc}[m]$\;
        $c_2 \gets T_{2,enc}[m]$\;
        $dist \gets dist + D[m, c_1, c_2]$\;
    }
    \Return{$\sqrt{dist}$}\;
}
\Fn{asymmetric($T_{1}$,\ $T_{2,enc}$, $C$) : $\mathbb{R}$}{
    $A \gets \emptyset$;
    \For{$m \gets 0$ \textbf{to} $M$} {
      $rs \gets m \times (D/M)$\;
      $re \gets rs + (D/M)$\;
      \For{$k \gets 0$ \textbf{to} $K$} {
         $A[m,k] \gets \textbf{dtw\_dist}(T_1[rs:re],\ C[m,k,:])$\;
      }
    }
    $dist \gets 0$\;
    \For{$m \gets 0$ \textbf{to} $M$} {
        $c_2 \gets T_{2,enc}[m]$\;
        $dist \gets dist + D[m, c_2]$\;
    }
    \Return{$\sqrt{dist}$}\;
}
 \caption{Distance estimation phase}
 \label{algo:distance}
\end{algorithm2e}

==> media/algo_encoding.tex <==
\begin{algorithm2e}[h]
\SetAlgoLined
\KwIn{\newline
$T$: The time series to encode $ \in \mathbb{R}^{D}$\newline
$C$: The codebook $\in \mathbb{R}^{M \times k \times D/M}$\newline
$E$: The Keogh envelopes $\in \mathbb{R}^{2 \times M \times k \times D/M}$
}
\KwOut{\newline
$T_{enc}$: The encoded time series $ \in \mathbb{N}^{M}$
}
 $T_{enc} \gets \emptyset$\;
\For{$m \gets 0$ \textbf{to} $M$} {
  $rs \gets m * (D/M)$\;
  $re \gets rs + (D/M)$\;
  $T_{enc}[m] \gets \textbf{1NN}(C[m, :, :], E[:, m, :, :], T[rs:re])$\;
}
  \SetKwProg{Fn}{Function}{ is}{end}
   \Fn{1NN(
       C: $\mathbb{R}^{k \times D/M}$,\ 
       E: $\mathbb{R}^{2 \times k \times D/M}$,\ 
       q: $\mathbb{R}^{D}$
   ) : $\mathbb{N}$}{
    $best\_so\_far \gets \infty$\; 
    \For{$i \gets 1$ \textbf{to} $|C|$}{
        $LB\_dist \gets \textbf{lower\_bound\_distance}(c_i, e_i, q)$\; 
        \If{$LB\_dist < best\_so\_far$}{
            $dist \gets \textbf{DTW}(c_i, q)$\;
            \If{$dist < best\_so\_far$}{
                $best\_so\_far \gets dist$\;
                $index\_of\_best\_match \gets i$\; 
            }
        }
    }
   \Return index\_of\_best\_match\;
   }
  \Return{$T_{enc}$}\;
 \caption{Encoding a time series}
\end{algorithm2e}

==> media/algo_training.tex <==
\begin{algorithm2e}[h]
\SetAlgoLined
\KwIn{\newline
$X$: The training data $ \in \mathbb{R}^{N \times D}$\newline
$M$: The number of sub-spaces\newline
$K$: The codebook size 
}
\KwOut{\newline
$C$: the codebook $\in \mathbb{R}^{M \times k \times D/M}$\newline
$D$: the distance lookup table $\in \mathbb{R}^{M \times k \times k}$\newline
$E$: the Keogh envelopes $\in \mathbb{R}^{2 \times M \times k \times D/M}$
}

    $C \gets \emptyset$; 
    $D \gets \emptyset$;
    $E \gets \emptyset$\;
    \For{$m \gets 0$ \textbf{to} $M$} {
      $rs \gets m \times (D/M)$\;
      $re \gets rs + (D/M)$\;
      $C[m,:,:] \gets \textbf{DBA\_kmeans}(X[:, rs:re],\ K)$\;
      \For{$k \gets 0$ \textbf{to} $K$} {
        \For{$l \gets 0$ \textbf{to} $K$} {
          $D[m,k,l] \gets \textbf{DTW}(C[m,k,:],\ C[m,l,:])$\;
         }
        $E[:,m,k,:] \gets \textbf{keogh\_envelope}(C[m,k,:])$\;
      }
    }
    \Return{$C$, $D$, $E$}\;
 \caption{Training phase}
 \label{algo:training}
\end{algorithm2e}
